Exact Convex Relaxation of Optimal Power Flow in Radial Networks

The optimal power flow (OPF) problem determines power generation/demand that minimize a certain objective such as generation cost or power loss. It is nonconvex. We prove that, for radial networks, after shrinking its feasible set slightly, the global optimum of OPF can be recovered via a second-order cone programming (SOCP) relaxation under a condition that can be checked a priori. The condition holds for the IEEE 13-, 34-, 37-, 123-bus networks and two real-world networks, and has a physical interpretation.

==> C1.tex <==
\subsection*{Proof for linear networks (Lemma \ref{lemma: line exact})}\label{app: line}
% Procedure
Assume the conditions in Lemma \ref{lemma: line exact} hold. If SOCP is not exact, then there exists an SOCP solution $w=(s,S,v,\ell,s_0)$ of SOCP that violates \eqref{Line 8}. Let
	\begin{equation}\label{m}
	m:=\min\left\{i\in \hN^+~\left|~\ell_i>|S_i|^2/v_i\right.\right\}
	\end{equation}
denote the first bus where \eqref{Line 8} is violated, then $m\in \hN^+$ and $\ell_m>|S_m|^2/v_m$. One can construct a point $w'=(s',S',v',\ell',s_0')$ according to Algorithm \ref{algorithm}.

	\begin{algorithm}
	\caption{Construct a point}
	\label{algorithm}
	\begin{algorithmic}[1]
    	\REQUIRE a feasible point $w=(s,S,v,\ell,s_0)$ of SOCP that violates \eqref{Line 8}, $m=\min\left\{i\in \hN^+~|~\ell_i>|S_i|^2/v_i\right\}$.
    	\ENSURE $w'=(s',S',v',\ell',s_0')$.
    	\STATE $s'\leftarrow s$;
	\STATE $S_n'\leftarrow s_n'$;
	\STATE $k\leftarrow n$;
	\WHILE{$k > 0$}
    		\STATE $\ell_k' \leftarrow \begin{cases}
			\ell_k & k>m, \\
			|S_k'|^2 / v_k & k\leq m;
			\end{cases}$
		\IF{$k\neq1$}
		\STATE $S_{k-1}'\leftarrow S_k'-z_k\ell_k'+s_{k-1}'$;
		\ELSE
		\STATE $s_0'\leftarrow z_1\ell_1' - S_1'$;
		\ENDIF
    	\ENDWHILE
	\STATE $v_0'\leftarrow v_0$;
	\STATE $k\leftarrow 1$;
	\WHILE{$k\leq n$}
	\STATE $v_k'\leftarrow v_{k-1}'+2\re(z_k^HS_k')-|z_k|^2\ell_k'$;
	\ENDWHILE
	\end{algorithmic}
	\end{algorithm}

% explain of the algorithm
Algorithm \ref{algorithm} keeps $s$ unchanged, i.e., $s'=s$, therefore $w'$ satisfies \eqref{Line 5}. The main step in Algorithm \ref{algorithm} is constructing $S'$, $\ell'$ and $s_0'$, after which $v'$ is simply constructed to satisfy \eqref{Line 4}. After initializing $S_n'=s_n'$ to satisfy \eqref{Line 1}, the construction of $\ell_k'$ and $S_{k-1}'$ (or $s_0'$) is done recursively for $k=n,\ldots,1$ as follows. First construct $\ell_k'$: keep $\ell_k'=\ell_k$ if $k>m$, and change $\ell_k$ to $\ell_k'=|S_k'|^2/v_k$ if $k\leq m$. After deciding on $\ell_k'$, the construction of $S_{k-1}'$/$s_0'$ is simply to satisfy \eqref{Line 2}/\eqref{Line 3}. Hence, $w'$ may only violate \eqref{Line 7} and \eqref{line relax} out of all the constraints in SOCP. It is not difficult to verify that $S_k'=S_k$ for $k\geq m$.



The following lemma provides a sufficient condition under which $w'$ is feasible for SOCP and has a smaller objective value than $w$. To state the lemma, let $S_0\eqdef -s_0$ denote the power that the substation injects to the main grid, and define
    $$\Delta S_i=\Delta P_i+\ii \Delta Q_i:=S_i'-S_i, \quad \Delta v_i:=v_i'-v_i$$
as the difference from $w'$ to $w$ for $i\in \hN$. Recall that $S_k'=S_k$ for $k\geq m$, therefore $\Delta S_k=0$ for $k\geq m$. For complex numbers, let the operators $<$, $\leq$, $>$, $\geq$ denote componentwise.

	\begin{lemma}\label{lemma: observation}
	Consider a linear network. Given a feasible point $w=(s,S,v,\ell,s_0)$ of SOCP that violates \eqref{Line 8}, let $m$ be defined as \eqref{m}, and $w'=(s',S',v',\ell',s_0')$ be the output of Algorithm \ref{algorithm}. If $\hat{v}_i(s)\leq \overline{v}_i$ for $i\in \hN^+$ and
	\begin{equation}\label{observation}
	S_k' > S_k \text{ for } 0\leq k\leq m-1,
	\end{equation}
then $w'$ is feasible for SOCP. If further, $f_0$ is strictly increasing, then $w'$ has a smaller objective value than $w$, i.e.,
    $$\sum_{i=0}^n f_i(\re(s_i')) < \sum_{i=0}^n f_i(\re(s_i)).$$
	\end{lemma}	
	
	\begin{proof}
	Assume that $\hat{v}_i(s)\leq\overline{v}_i$ for $i\in\hN^+$ and $\Delta S_k>0$ for $0\leq k\leq m-1$. To check $w'$ is feasible for SOCP, it suffices to show that $w'$ satisfies \eqref{Line 7} and \eqref{line relax}, i.e., $\underline{v}_i\leq v_i'\leq\overline{v}_i$ and $\ell_i'\geq |S_i'|^2/v_i'$ for $i\in\hN^+$. Since $w'$ satisfies \eqref{BFM S}--\eqref{BFM v} and $\ell'\geq0$, one has $v_i'\leq \hat{v}_i(s') =\hat{v}_i(s) \leq \overline{v}_i$ for $i\in \hN^+$ according to Lemma \ref{lemma: v}. Note that $\Delta S_k=0$ for $m\leq k\leq n$. Then, it follows from \eqref{Line 2} and \eqref{Line 4} that
	$\Delta v_i - \Delta v_{i-1} = \re ( z_i^H \Delta S_i) + \re ( z_i^H \Delta S_{i-1}) \geq 0$
for $i \in \hN^+$ and the inequality is strict for $1\leq i\leq m$. Hence,
	$\Delta v_n \geq \ldots \geq \Delta v_m > \Delta v_{m-1} >\ldots >  \Delta v_0=0$,
which implies $v_i'> v_i\geq\underline{v}_i$ for $i\in \hN^+$. One has $\ell_i'=\ell_i\geq|S_i|^2/v_i=|S_i'|^2/v_i\geq|S_i'|^2/v_i'$ for $i>m$ and $\ell_i' = |S_i'|^2/v_i \geq |S_i'|^2/v_i'$ for $i\leq m$. Hence, $w'$ is feasible for SOCP.

If further, $f_0$ is strictly increasing, then
	$\sum_{i=0}^n f_i(\re(s_i')) - \sum_{i=0}^n f_i(\re(s_i))
	%= f_0(\re(s_0')) - f_0(\re(s_0))
    	= f_0(-\re(S_0')) - f_0(-\re(S_0)) < 0,$
i.e., $w'$ has a smaller objective value than $w$. This completes the proof of Lemma \ref{lemma: observation}.
	\end{proof}
	
	
	
	
	
	\begin{remark}
We illustrate that \eqref{observation} seems natural to hold with Fig. \ref{fig: illustrate}.	
	\begin{figure}[!htbp]
     	\centering
     	\includegraphics[scale=0.25]{illustration}
      	\caption{Illustration of \eqref{observation}.}
      	\label{fig: illustrate}
	\end{figure}
Recall that $S_m'=S_m$ and $\ell_m'=|S_m'|^2/v_m = |S_m|^2/v_m < \ell_m$. Define $\epsilon:=\ell_m-\ell_m'>0$, then
	\begin{eqnarray}
	\Delta S_{m-1} = \Delta S_m-z_m\Delta\ell_m = z_m\epsilon > 0. \label{m difference}
	\end{eqnarray}
Intuitively, after increasing $S_{m-1}$, upstream power flow ($S_k$ for $0\leq k\leq m-2$) is likely to increase. Lemma \ref{lemma: observation} says that if upstream power flow indeed increases, then $w'$ is feasible and ``better'' than $w$.
\end{remark}

% importance
%Assume that $f_0$ is strictly increasing. Lemma \ref{lemma: observation} implies that for any optimal solution $w=(s,S,v,\ell,s_0)$ of SOCP, if $\hat{v}_i(s)\leq \overline{v}_i$ for $i\in \hN^+$ and there exists some $\epsilon\in(0,\ell_m-|S_m|^2/v_m]$ such that $w'(\epsilon)$ satisfies \eqref{observation}, then $w$ cannot be optimal for SOCP, which is a contradiction.


%%%%%%%%%%%%%%%%%%%%%
%\subsection*{Step (S3)}
% motivate linearization
Now we compute $\Delta S_k$ for $0\leq k\leq m-1$. For any $t\in\{1,\ldots,m-1\}$, one has
	\begin{eqnarray*}
	\Delta \ell_t = \frac{P_t'^2+Q_t'^2}{v_t}-\frac{P_t^2+Q_t^2}{v_t}
	= \frac{2P_t''\Delta P_t}{v_t} +\frac{2Q_t''\Delta Q_t}{v_t}
	\end{eqnarray*}
where $P_t''=(P_t+P_t')/2$ and $Q_t''=(Q_t+Q_t')/2$. Hence,
	\begin{eqnarray*}
	(\Delta P_{t-1}, \Delta Q_{t-1})^T =
	(\Delta P_t, \Delta Q_t)^T
	-( r_t, x_t)^T \Delta \ell_t
	= A_t
	(\Delta P_t, \Delta Q_t)^T\label{recursive}
	\end{eqnarray*}
where
	$$A_t = \begin{pmatrix} 1-\frac{2r_tP_t''}{v_t} & -\frac{2r_tQ_t''}{v_t}\\ -\frac{2x_tP_t''}{v_t} & 1-\frac{2x_tQ_t''}{v_t} \end{pmatrix}$$
for $t=1,\ldots,m-1$. It follows from \eqref{m difference} that $(\Delta P_{m-1}, \Delta Q_{m-1})^T = u_m \epsilon$, therefore $\Delta S_k$ for $0\leq k\leq m-1$ can be computed as in the following lemma.

    \begin{lemma}\label{lemma: Taylor}
    Consider a linear network. Given a feasible point $w=(s,S,v,\ell,s_0)$ of SOCP that violates \eqref{Line 8}, let $m$ be defined as \eqref{m}, and $w'=(s',S',v',\ell',s_0')$ be the output of Algorithm \ref{algorithm}. Then
	\begin{equation}\label{Taylor}
	(\Delta P_{t-1}, \Delta Q_{t-1})^T = A_t\cdots A_{m-1}u_m\epsilon
	\end{equation}
for $t=1,\ldots,m$.
    \end{lemma}
At last, we show that \eqref{C1 line} implies $\Delta S_k>0$ for $0\leq k\leq m-1$. It suffices to prove that $\underline{A}_t\cdots \underline{A}_{s-1}u_s>0$ for $1\leq t\leq s \leq m$ implies $A_t\cdots A_{s-1}u_s>0$ for $1\leq t\leq s\leq m$. To prove this, we need the following lemma.

	\begin{lemma}\label{lemma: dynamical system}
	Given $m\geq1$ and $d\geq1$. Let $\underline{A}_1,\ldots,\underline{A}_{m-1}, A_1,\ldots,A_{m-1}\in\mathbb{R}^{d\times d}$ 	and $u_1,\ldots,u_m\in\mathbb{R}^d$ satisfy
	\begin{itemize}
	\item $\underline{A}_t\cdots \underline{A}_{s-1}u_s>0$ for $1\leq t\leq s \leq m$;
	\item there exists $b_t\in\mathbb{R}^d$ that satisfies $b_t\geq0$ and $A_t-\underline{A}_t=u_tb_t^T$, for $t=1,\ldots,m-1$.
	\end{itemize}
	Then 
	\begin{equation}\label{dynamical}
	A_t\cdots A_{s-1}u_s>0
	\end{equation}
	for $1\leq t\leq s \leq m$.
	\end{lemma}

\begin{proof}
We prove that \eqref{dynamical} holds for $1\leq t\leq s\leq m$ by mathematical induction on $s-t$.
\begin{itemize}
\item[i)] When $s-t=0$, one has
    $A_t\cdots A_{s-1}u_s = u_s = \underline{A}_t\cdots \underline{A}_{s-1}u_s > 0.$
\item[ii)] Assume that \eqref{dynamical} holds for $s-t\leq K$ ($0\leq K\leq m-2$). When $s-t=K+1$, one has
    \begin{eqnarray*}
    A_t\cdots A_k\underline{A}_{k+1}\cdots \underline{A}_{s-1}u_s
    &=& A_t\cdots A_{k-1}\underline{A}_{k}\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s 
    + A_t\cdots A_{k-1}(A_k-\underline{A}_{k})\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s\\
    &=& A_t\cdots A_{k-1}\underline{A}_{k}\cdots \underline{A}_{s-1} u_s 
    + A_t\cdots A_{k-1}u_kb_k^T\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s\\
    &=& A_t\cdots A_{k-1}\underline{A}_{k}\cdots \underline{A}_{s-1} u_s 
    + \left(b_k^T\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s\right)A_t\cdots A_{k-1}u_k
    \end{eqnarray*}
whenever $t \leq k < s$. Since $b_k\geq0$ and $\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s>0$, the term $b_k^T\underline{A}_{k+1}\cdots \underline{A}_{s-1} u_s\geq0$. According to induction hypothesis, $A_t\cdots A_{k-1} u_k>0$. Hence,
   \begin{eqnarray*}
    A_t\cdots A_k\underline{A}_{k+1}\cdots \underline{A}_{s-1}u_s
    \geq A_t\cdots A_{k-1}\underline{A}_{k}\cdots \underline{A}_{s-1} u_s
    \end{eqnarray*}
whenever $t\leq k<s$. By substituting $k=s-1,\ldots,t$ in turn, one obtains
    \begin{eqnarray*}
    A_t\cdots A_{s-1}u_s
    \geq A_t\cdots A_{s-2}\underline{A}_{s-1}u_s
    \geq \cdots \geq \underline{A}_t \cdots \underline{A}_{s-1} u_s > 0,
    \end{eqnarray*}
i.e., \eqref{dynamical} holds for $s-t=K+1$.
\end{itemize}
According to (i) and (ii), \eqref{dynamical} holds for $s-t=0,\ldots,m-1$. This completes the proof of Lemma \ref{lemma: dynamical system}.
\end{proof}

\begin{lemma}\label{lemma: increase}
Consider a linear network. Given a feasible point $w=(s,S,v,\ell,s_0)$ of SOCP that violates \eqref{Line 8}, let $m$ be defined as \eqref{m}, and $w'=(s',S',v',\ell',s_0')$ be the output of Algorithm \ref{algorithm}. If \eqref{C1 line} holds, then $\Delta S_k > 0$ for $0\leq k\leq m-1$.
\end{lemma}

\begin{proof}
When \eqref{C1 line} holds, $\underline{A}_t\cdots \underline{A}_{s-1}u_s>0$ for $1\leq t\leq s \leq m$. Note that
	$$A_t-\underline{A}_t=u_t\left(\frac{2}{\underline{v}_t}\hat{P}_t^+(\overline{p})-\frac{2}{v_t}P_t'',  ~\frac{2}{\underline{v}_t}\hat{Q}_t^+(\overline{q})-\frac{2}{v_t}Q_t''\right)^T$$
where $b_t=(2/\underline{v}_t-2/v_t)\left(\hat{P}_t^+(\overline{p}), \hat{Q}_t^+(\overline{q})\right)^T\geq0$ for $t=1,\ldots,m-1$.
According to Lemma \ref{lemma: dynamical system}, one has
	$$\begin{pmatrix} 1-\frac{2r_t\hat{P}^+_t(\overline{p})}{v_t} & -\frac{2r_t\hat{Q}_t^+(\overline{q})}{v_t}\\ -\frac{2x_t\hat{P}_t^+(\overline{p})}{v_t} & 1-\frac{2x_t\hat{Q}_t^+(\overline{q})}{v_t}\end{pmatrix}\cdots
	\begin{pmatrix} 1-\frac{2r_{s-1}\hat{P}^+_{s-1}(\overline{p})}{v_{s-1}} & -\frac{2r_{s-1}\hat{Q}_{s-1}^+(\overline{q})}{v_{s-1}}\\ -\frac{2x_{s-1}\hat{P}_{s-1}^+(\overline{p})}{v_{s-1}} & 1-\frac{2x_{s-1}\hat{Q}_{s-1}^+(\overline{q})}{v_{s-1}}\end{pmatrix}u_s>0$$
for $1\leq t\leq s\leq m$.

Now, let $M_t=A_t$ for $t=1,\ldots,m-1$, let
	$$\underline{M}_t=\begin{pmatrix} 1-\frac{2r_t\hat{P}^+_t(\overline{p})}{v_t} & -\frac{2r_t\hat{Q}_t^+(\overline{q})}{v_t}\\ -\frac{2x_t\hat{P}_t^+(\overline{p})}{v_t} & 1-\frac{2x_t\hat{Q}_t^+(\overline{q})}{v_t}\end{pmatrix}$$
for $t=1,\ldots,m-1$, and let $w_t=u_t$ for $t=1,\ldots,m$, then
	\begin{itemize}
	\item $\underline{M}_t\cdots \underline{M}_{s-1}w_s=\begin{pmatrix} 1-\frac{2r_t\hat{P}^+_t(\overline{p})}{v_t} & -\frac{2r_t\hat{Q}_t^+(\overline{q})}{v_t}\\ -\frac{2x_t\hat{P}_t^+(\overline{p})}{v_t} & 1-\frac{2x_t\hat{Q}_t^+(\overline{q})}{v_t}\end{pmatrix}\cdots
	\begin{pmatrix} 1-\frac{2r_{s-1}\hat{P}^+_{s-1}(\overline{p})}{v_{s-1}} & -\frac{2r_{s-1}\hat{Q}_{s-1}^+(\overline{q})}{v_{s-1}}\\ -\frac{2x_{s-1}\hat{P}_{s-1}^+(\overline{p})}{v_{s-1}} & 1-\frac{2x_{s-1}\hat{Q}_{s-1}^+(\overline{q})}{v_{s-1}}\end{pmatrix}u_s>0$ for $1\leq t\leq s \leq m$;
	\item $M_t-\underline{M}_t=u_tb_t^T$ where $b_t=2/v_t\left(\hat{P}_t^+(\overline{p})-P_t'', \hat{Q}_t^+(\overline{q})-Q_t''\right)^T$ for $t=1,\ldots,m-1$.
	\end{itemize}
Since $w$ and $w'$ both satisfy \eqref{BFM S}--\eqref{BFM v} and $\ell,\ell'\geq0$, one has
	$$S_t\leq \hat{S}_t(s), ~S_t'\leq\hat{S}_t(s')=\hat{S}_t(s)$$
for $t=1,\ldots,m-1$. It follows that $S_t''=(S_t+S_t')/2\leq \hat{S}_t(s)$ for $t=1,\ldots,m-1$. Hence, $P_t''\leq\hat{P}_t({p})\leq\hat{P}_t(\overline{p})\leq\hat{P}_t^+(\overline{p})$ and $Q_t''\leq\hat{Q}_t({q})\leq\hat{Q}_t(\overline{q})\leq\hat{Q}_t^+(\overline{q})$ for $t=1,\ldots,m-1$. This implies that $b_t\geq0$ for $t=1,\ldots,m-1$. According to Lemma \ref{lemma: dynamical system}, one has $M_t\cdots M_{s-1}w_s = A_t\cdots A_{s-1}u_s >0$ for $1\leq t\leq s\leq m$.

At last, according to Lemma \ref{lemma: Taylor}, one has $(\Delta P_{t-1}, \Delta Q_{t-1})^T = A_t\cdots A_{m-1}u_m\epsilon>0$ for $t=1,\ldots,m$. This completes the proof of Lemma \ref{lemma: increase}.
\end{proof}

Now we come back to the proof of Lemma \ref{lemma: line exact}. Assume the conditions in Lemma \ref{lemma: line exact} hold, then the conditions in Lemma \ref{lemma: increase} hold and therefore $\Delta S_k>0$ for $0\leq k\leq m-1$. Then, the conditions in Lemma \ref{lemma: observation} hold, and it follows that $w'$ has a smaller objective value than $w$. This contradicts with $w$ being optimal for SOCP, and completes the proof of Lemma \ref{lemma: line exact}.

